Putting Transformer Theories to the Test

Several formal theories have been developed to characterize the capabilities and limitations of the transformer architecture, each employing different abstractions that capture different features of the architecture. Due to the differences in their underlying assumptions and conceptual frameworks, these theories can disagree in their predictions about what tasks transformers find easy or hard. We map out seven theories of transformer capability (Star-free, $\mathsf{AC}^0$, $\mathsf{TC}^0$, C-RASP, MPC, BAPO, and Sensitivity) and translate their results into a common matrix of predictions across a suite of tasks covering different computational structures. We provide new theoretical results to complete this matrix. We then evaluate theoretical predictions through controlled experiments measuring in-distribution sample complexity, length generalization, and pretrained language model performance. We find that no single theory explains the observed pattern of successes and failures. When a theory does not capture the transformer behaviors relevant to a task, its predictions break down; for instance, we show that the $k$-hop induction task is predicted hard by C-RASP because it does not model content-dependent attention, but we train small transformers on this task that length-generalize. Similarly, theories assuming hard attention like $\mathsf{AC}^0$ and BAPO predict binary majority to be hard, for which we also find success in practice. Together, our results point to several specific features that a theory of transformers must capture: soft rather than hard attention, dynamic content-dependent retrieval, bounded computation at each position, an account of learnability and inductive biases, and a combination of upper and lower bounds.

==> figure-generation/diagrams/theory-venn-diagram/figure-style.tex <==
\ifx\VennTheoryColour\undefined\def\VennTheoryColour{0}\fi
\ifx\VennFills\undefined\def\VennFills{1}\fi
\ifnum\VennTheoryColour=2
  \definecolor{vennink}{HTML}{263544}
  \definecolor{vennsfline}{HTML}{087E9A}
  \definecolor{vennsffill}{HTML}{E8F5F7}
  \definecolor{vennacline}{HTML}{246FB1}
  \definecolor{vennacfill}{HTML}{EAF2FA}
  \definecolor{venntcline}{HTML}{5B59A0}
  \definecolor{venntcfill}{HTML}{F0EFF8}
  \definecolor{venncountline}{HTML}{287B64}
  \definecolor{venncountfill}{HTML}{EAF4EE}
  \definecolor{vennmpcline}{HTML}{263C68}
  \definecolor{vennmpcfill}{HTML}{F0F2F7}
  \definecolor{vennbapoline}{HTML}{A64E73}
  \definecolor{vennbapofill}{HTML}{F7EBF0}
\else
  \definecolor{vennink}{HTML}{2F4858}
  \definecolor{vennsfline}{HTML}{B4508A}
  \definecolor{vennsffill}{HTML}{F2E0EA}
  \definecolor{vennacline}{HTML}{1B7F8E}
  \definecolor{vennacfill}{HTML}{D6E8EB}
  \definecolor{venntcline}{HTML}{8E56A6}
  \definecolor{venntcfill}{HTML}{EBE1EF}
  \definecolor{venncountline}{HTML}{2F6FB3}
  \definecolor{venncountfill}{HTML}{DAE5F1}
  \definecolor{vennmpcline}{HTML}{5D53A8}
  \definecolor{vennmpcfill}{HTML}{E2E0EF}
  \definecolor{vennbapoline}{HTML}{5A6472}
  \definecolor{vennbapofill}{HTML}{E1E3E6}
\fi

\tikzset{
  venn region/.style={draw=vennink,line width=.7pt,rounded corners=7pt},
  venn bapo/.style={venn region},
  venn mpc/.style={venn region},
  venn name/.style={anchor=north west,inner sep=0pt,font=\footnotesize},
  venn task/.style={circle,draw=vennink,fill=vennink,line width=.55pt,
    inner sep=0pt,minimum size=1.55mm},
  venn task open/.style={venn task,fill=white},
  venn task name/.style={font=\fontsize{7.5}{8.5}\selectfont,
    inner sep=0pt,text=vennink},
}


==> figure-generation/diagrams/theory-venn-diagram/horizontal/figure-body.tex <==
\ifx\VennTheoryColour\undefined\def\VennTheoryColour{0}\fi

\begin{tikzpicture}[x=1cm,y=1cm]
\input{figure-generation/diagrams/theory-venn-diagram/figure-style.tex}%
\path[use as bounding box] (0,0) rectangle (14.56,4.56);

\def\rowCR{1.45} \def\rowSF{2.22} \def\rowArm{3.08}
\def\mpcSW{(0.08,0.08)} \def\mpcNE{(12.41,4.48)}
\def\tcSW{(0.30,0.30)}  \def\tcNE{(9.85,4.20)}
\def\acSW{(0.52,0.52)}  \def\acNE{(6.68,3.92)}
\def\sfSW{(0.86,0.86)}  \def\sfNE{(4.60,2.62)}
\def\tlSW{(1.05,1.12)}  \def\tlNE{(9.67,1.78)}

\def\bapoPath{%
  (14.48,2.80) -- (4.77,2.80) -- (4.77,0.70) --
  (0.70,0.70) -- (0.70,3.36) -- (14.48,3.36) -- cycle}

\ifnum\VennTheoryColour>0
  \colorlet{mpcedge}{vennmpcline}    \colorlet{mpcname}{vennmpcline}
  \colorlet{tcedge}{venntcline}      \colorlet{tcname}{venntcline}
  \colorlet{acedge}{vennacline}      \colorlet{acname}{vennacline}
  \colorlet{sfedge}{vennsfline}      \colorlet{sfname}{vennsfline}
  \colorlet{tledge}{venncountline}   \colorlet{tlname}{venncountline}
  \colorlet{bapoedge}{vennbapoline} \colorlet{baponame}{vennbapoline}
  \ifnum\VennFills=1
  \path[fill=vennmpcfill,even odd rule,rounded corners=5pt]
    \mpcSW rectangle \mpcNE \tcSW rectangle \tcNE;
  \path[fill=venntcfill,even odd rule,rounded corners=5pt]
    \tcSW rectangle \tcNE \acSW rectangle \acNE;
  \path[fill=vennacfill,even odd rule,rounded corners=5pt]
    \acSW rectangle \acNE \sfSW rectangle \sfNE;
  \path[fill=vennsffill,rounded corners=5pt] \sfSW rectangle \sfNE;
  \path[fill=vennbapofill,fill opacity=.42,rounded corners=5pt] \bapoPath;
  \path[fill=venncountfill,fill opacity=.42,rounded corners=5pt]
    \tlSW rectangle \tlNE;
  \fi
\else
  \colorlet{mpcedge}{vennink} \colorlet{mpcname}{vennink}
  \colorlet{tcedge}{vennink}  \colorlet{tcname}{vennink}
  \colorlet{acedge}{vennink}  \colorlet{acname}{vennink}
  \colorlet{sfedge}{vennink}  \colorlet{sfname}{vennink}
  \colorlet{tledge}{vennink}  \colorlet{tlname}{vennink}
  \colorlet{bapoedge}{vennink}\colorlet{baponame}{vennink}
  \ifnum\VennFills=1
  \path[fill=vennink,fill opacity=.035,rounded corners=5pt]
    \mpcSW rectangle \mpcNE;
  \path[fill=vennink,fill opacity=.045,rounded corners=5pt]
    \tcSW rectangle \tcNE;
  \path[fill=vennink,fill opacity=.045,rounded corners=5pt]
    \acSW rectangle \acNE;
  \path[fill=vennink,fill opacity=.045,rounded corners=5pt]
    \sfSW rectangle \sfNE;
  \path[fill=vennink,fill opacity=.055,rounded corners=5pt] \bapoPath;
  \path[fill=vennink,fill opacity=.055,rounded corners=5pt]
    \tlSW rectangle \tlNE;
  \fi
\fi

\tikzset{
  venn landscape region/.style={draw=vennink,line width=.6pt,rounded corners=5pt},
  venn landscape cross/.style={venn landscape region,line width=.8pt},
  venn landscape name/.style={inner sep=0pt,font=\fontsize{7.5}{8.5}\selectfont},
  venn landscape task/.style={circle,draw=vennink,fill=vennink,line width=.5pt,
    inner sep=0pt,minimum size=1.3mm},
  venn landscape task open/.style={venn landscape task,fill=white},
  venn landscape task name/.style={font=\fontsize{6.5}{7.3}\selectfont,
    inner sep=0pt,text=vennink,anchor=west,align=left},
}

\draw[venn landscape region,draw=mpcedge] \mpcSW rectangle \mpcNE;
\draw[venn landscape region,draw=tcedge] \tcSW rectangle \tcNE;
\draw[venn landscape region,draw=acedge] \acSW rectangle \acNE;
\draw[venn landscape region,draw=sfedge] \sfSW rectangle \sfNE;
\draw[venn landscape cross,draw=tledge] \tlSW rectangle \tlNE;
\draw[venn landscape cross,draw=bapoedge] \bapoPath;

\node[venn landscape name,anchor=north east,text=mpcname] at (12.29,4.38) {\MPC};
\node[venn landscape name,anchor=north east,text=tcname] at (9.73,4.10) {$\TCz$};
\node[venn landscape name,anchor=north east,text=acname] at (6.56,3.82) {$\ACz$};
\node[venn landscape name,anchor=west,text=sfname] at (0.98,\rowSF) {\Starfree};
\node[venn landscape name,anchor=west,text=baponame] at (0.84,\rowArm) {\BAPO};
\node[venn landscape name,anchor=west,text=tlname] at (1.17,\rowCR) {\CRASP};

\newcommand{\venntask}[4][venn landscape task]{%
  \node[#1] at (#2,#3) {};
  \node[venn landscape task name] at ({#2+0.12},#3) {#4};}

\venntask{2.35}{\rowCR}{\TaskALL}
\venntask{3.05}{\rowCR}{\TaskANY}
\venntask{2.20}{\rowSF}{\TaskKHop}
\venntask{5.05}{\rowArm}{\TaskIndex}
\venntask{4.97}{\rowSF}{\TaskBinaryAddition}

\venntask{6.96}{\rowArm}{\TaskParity}
\venntask{6.96}{\rowSF}{\TaskDyckTwo}
\venntask{6.96}{\rowCR}{\TaskDyckOne}
\venntask{8.15}{\rowCR}{\TaskMajority}

\venntask[venn landscape task open]{10.13}{\rowArm}{$S_5$ word problem}
\venntask[venn landscape task open]{10.13}{\rowCR}{Boolean formula\\value problem}
\venntask[venn landscape task open]{12.69}{\rowSF}{\taskname{Reachability}}

\end{tikzpicture}


==> figures/diagrams/theory-transformer-relations/theory-transformer-relation-body.tex <==
\begin{tikzpicture}[x=1cm,y=1cm]
\def\cA{1.35}\def\cB{4.50}\def\cC{7.65}\def\cD{10.80}\def\cE{13.95}
\def\rowM{-2.15}
\ifnum\RelationsShowSources=1
  \ifnum\RelationsFooterMerge=1 \def\relbottom{-4.08}\else\def\relbottom{-4.42}\fi
\else
  \def\relbottom{-2.62}
\fi
\path[use as bounding box] (.05,\relbottom) rectangle (15.25,1.22);

\node[rel legend] at (.15,1.02) {$A$};
\draw[rel yes] (.45,1.02) -- (1.05,1.02);
\node[rel legend] at (1.15,1.02) {$B$\,: \ $A \subseteq B$};
\node[rel legend] at (3.25,1.02) {$A$};
\draw[rel no] (3.55,1.02) -- (4.15,1.02);
\node[rel legend] at (4.25,1.02) {$B$\,: \ $A \nsubseteq B$};
\draw[rel yes,rel dashed,draw=relink] (6.55,1.02) -- (7.15,1.02);
\node[rel legend] at (7.27,1.02) {\RelationsDashedLabel};

\node[rel theory] (sf) at (\cA,0) {\Starfree};
\node[rel theory] (ac) at (\cB,0) {\textbf{\boldmath\ACz}};
\node[rel theory] (tc) at (\cC,0) {\textbf{\boldmath\TCz}};
\node[rel theory] (mpc) at (\cD,0) {\MPC};
\node[rel theory] (cr) at (\cE,0) {\CRASP};

\node[rel model] (hd) at (\cA,\rowM) {Causal\\Hard Attn.};
\node[rel model] (he) at (\cB,\rowM) {Bidirectional\\Hard Attn.};
\node[rel model] (ae) at (\cC,\rowM) {Bidirectional\\Avg.-Hard Attn.};
\node[rel model] (se) at (\cD,\rowM) {Bidirectional\\Softmax Attn.};
\node[rel model] (sd) at (\cE,\rowM) {Causal\\Softmax Attn.};

\path let \p1=(sf.south), \p2=(hd.north) in \pgfextra{%
  \pgfmathsetlengthmacro{\relkeyrowtmp}{(\y1+\y2)/2}\global\let\relkeyrow\relkeyrowtmp
  \pgfmathsetlengthmacro{\relslashrowtmp}{(\y1+3*\y2)/4}\global\let\relslashrow\relslashrowtmp};

\draw[rel yes] (sf.east) -- (ac.west);
\draw[rel yes] (ac.east) -- (tc.west);
\draw[rel yes] (tc.east) -- (mpc.west);
\draw[rel yes] (cr.west) -- (mpc.east);
\draw[rel yes,rounded corners=4pt] ([xshift=-14pt]cr.north) -- ++(0,.3) -| ([xshift=14pt]tc.north);

\relpair[5]{sf.south}{hd.north}{rel yes,rel dashed}{relyes}{a}{rel yes}{relyes}{b}
\relpair{[xshift=18pt]sf.south}{[xshift=-26pt]he.north}{rel yes}{relyes}{c}{rel no}{relno}{d}
\relpair[5]{ac.south}{he.north}{rel no}{relno}{e}{rel yes}{relyes}{f}
\relone{rel no}{relno}{[xshift=-26pt]ae.north}{[xshift=18pt]ac.south}{g}
\relpair[5]{tc.south}{ae.north}{rel no,rel dashed}{relno}{h}{rel yes}{relyes}{i}
\relpair{[xshift=18pt]tc.south}{[xshift=-26pt]se.north}{rel no,rel dashed}{relno}{j}{rel yes}{relyes}{k}
\relpair[5]{mpc.south}{se.north}{rel yes,rel dashed}{relyes}{m}{rel yes}{relyes}{n}

\relarrow{rel yes}{relyes}{[xshift=-10pt]cr.south}{[xshift=-10pt]sd.north}{o}{left}
\relarrow{rel yes,rel dashed}{relyes}{sd.north}{cr.south}{p}{right}
\relarrow{rel no,rel dashed}{relno}{[xshift=10pt]sd.north}{[xshift=10pt]cr.south}{q}{right}

\ifnum\RelationsShowSources=1
  \newcommand{\relsources}[2]{%
    \draw[relink!18,line width=.4pt] ({#1-1.3},-2.82) -- ({#1+1.3},-2.82);
    \node[anchor=north,inner sep=0pt,text=relink,font=\sffamily\fontsize{7.5}{9.6}\selectfont]
      at (#1,-2.98) {\begin{tabular}{@{}l@{\hspace{.4em}}l@{}}#2\end{tabular}};}
  \ifnum\RelationsFooterMerge=1
    \relsources{\cA}{%
      \textbf{a, b} & \relref{YCA24}{yang2024masked}{Th.~5} \\
      \textbf{c} & \relref{B+24}{barcelo2024logical}{Th.~1} \\
      \textbf{d} & \relref{B+24}{barcelo2024logical}{Cor.~1}}
  \else
    \relsources{\cA}{%
      \textbf{a} & \relref{YCA24}{yang2024masked}{Th.~5} \\
      \textbf{b} & \relref{YCA24}{yang2024masked}{Th.~5} \\
      \textbf{c} & \relref{B+24}{barcelo2024logical}{Th.~1} \\
      \textbf{d} & \relref{B+24}{barcelo2024logical}{Cor.~1}}
  \fi
  \relsources{\cB}{%
    \textbf{e} & \relref{B+24}{barcelo2024logical}{Prop.~1} \\
    \textbf{f} & \relref{HAF22}{hao2022formal}{Th.~1} \\
    \textbf{g} & \relref{B+24}{barcelo2024logical}{Cor.~2}}
  \ifnum\RelationsFooterMerge=1
    \relsources{\cC}{%
      \textbf{h, j} & \relref{MS23}{merrill2023logic}{}; \relref{SMCS26}{svete2026padded}{} \\
      \textbf{i} & \relref{S23}{strobl2023average}{Th.~2} \\
      \textbf{k} & \relref{MS23}{merrill2023logic}{Th.~2}}
  \else
    \relsources{\cC}{%
      \textbf{h} & \relref{MS23}{merrill2023logic}{}; \relref{SMCS26}{svete2026padded}{} \\
      \textbf{i} & \relref{S23}{strobl2023average}{Th.~2} \\
      \textbf{j} & \relref{MS23}{merrill2023logic}{}; \relref{SMCS26}{svete2026padded}{} \\
      \textbf{k} & \relref{MS23}{merrill2023logic}{Th.~2}}
  \fi
  \relsources{\cD}{%
    \textbf{m} & \relref{SHT24}{sanford2024parallel}{Th.~3.1} \\
    \textbf{n} & \relref{SHT24}{sanford2024parallel}{Th.~3.4}}
  \relsources{\cE}{%
    \textbf{o} & \relref{YC24}{yang2024counting}{Th.~5.7} \\
    \textbf{p} & \relref{YC24}{yang2024counting}{Th.~7.1} \\
    \textbf{q} & \relownref}
\fi
\end{tikzpicture}%


==> figures/diagrams/theory-transformer-relations/theory-transformer-relation-style.tex <==

\ifx\RelationsShowSources\undefined\def\RelationsShowSources{0}\fi
\ifx\RelationsKeySmall\undefined\def\RelationsKeySmall{0}\fi
\ifx\RelationsFooterMerge\undefined\def\RelationsFooterMerge{0}\fi
\ifx\RelationsKeyInline\undefined\def\RelationsKeyInline{0}\fi

\ifnum\RelationsSlash=0
  \ifnum\RelationsColorArrows=0
    \PackageError{theory-transformer-relations}{%
      \string\RelationsSlash\space and \string\RelationsColorArrows\space are both 0}{%
      Non-containment arrows would look the same as containment arrows.
      Set at least one of the two options to 1.}
  \fi
\fi

\providecommand{\RelationsDashedLabel}{with caveats}

\providecommand{\relref}[3]{#1\if\relax\detokenize{#3}\relax\else, #3\fi}
\providecommand{\relownref}{Ours}

\RelationsSetColors

\ifnum\RelationsKeySmall=1
  \def\relkeyfont{\sffamily\bfseries\fontsize{6}{7}\selectfont}
\else
  \def\relkeyfont{\sffamily\bfseries\fontsize{7}{8}\selectfont}
\fi
\tikzset{
  rel theory/.style={draw=relink,text=relink,rounded corners=6pt,minimum width=2.1cm,
    minimum height=.5cm,inner xsep=5pt,inner ysep=2pt,line width=.6pt,
    font=\sffamily\bfseries\fontsize{9.5}{11.5}\selectfont},
  rel model/.style={rounded corners=2pt,fill=relink!6,text=relink,text width=2.45cm,
    minimum height=.8cm,align=center,inner xsep=3pt,inner ysep=3pt,
    font=\sffamily\fontsize{8.5}{10.2}\selectfont},
  rel base/.style={line width=.7pt,shorten <=.6pt,shorten >=.6pt,
    -{Stealth[length=4.2pt,width=3.4pt]}},
  rel yes/.style={rel base,draw=relyes},
  rel dashed/.style={dash pattern=on 2.6pt off 1.9pt},
  rel key/.style={inner sep=1.2pt,font=\relkeyfont},
  rel legend/.style={anchor=west,inner sep=0pt,text=relink,
    font=\sffamily\fontsize{8.5}{10}\selectfont},
}
\ifnum\RelationsSlash=1
  \tikzset{rel no/.style={rel base,draw=relno,postaction={decorate},decoration={markings,
    mark=at position \relslashpos with {%
      \draw[-,relno,line width=.7pt,solid] (-3.2pt,0) -- (3.2pt,0);%
      \draw[-,relno,line width=.9pt,solid] (-1.5pt,-2.8pt) -- (1.5pt,2.8pt);}}}}
\else
  \tikzset{rel no/.style={rel base,draw=relno}}
\fi
\ifnum\RelationsShowSources=1
  \tikzset{rel key inline/.style={fill=white,inner xsep=.9pt,inner ysep=1.8pt}}
\else
  \tikzset{rel key inline/.style={}}
\fi

\def\relslashpos{.6}
\providecommand{\hyperlink}[2]{#2}
\newcommand{\relkeytext}[1]{\ifnum\RelationsShowSources=1 %
  \colorlet{relkeycolor}{.}\hyperlink{rel-edge-#1}{\textcolor{relkeycolor}{#1}}\fi}
\def\relrowanchorleft{mid east}
\def\relrowanchorright{mid west}
\def\relrowsignleft{-}
\def\relrowsignright{}
\newcommand{\relarrow}[6]{%
  \coordinate (relarrow-from) at (#3);
  \coordinate (relarrow-to) at (#4);
  \path let \p1=(relarrow-from), \p2=(relarrow-to),
    \p3=(0pt,\relkeyrow), \p4=(0pt,\relslashrow) in \pgfextra{%
      \pgfmathparse{(\y3-\y1)/(\y2-\y1)}\xdef\relrowkeypos{\pgfmathresult}%
      \pgfmathparse{(\y4-\y1)/(\y2-\y1)}\xdef\relrowslashpos{\pgfmathresult}%
      \pgfmathparse{.35+3.3*abs((\x2-\x1)/(\y2-\y1))}\xdef\relrowgap{\pgfmathresult pt}};
  \begingroup
  \let\relslashpos\relrowslashpos
  \draw[#1] (relarrow-from) -- (relarrow-to);
  \coordinate (relarrow-key) at ($(relarrow-from)!\relrowkeypos!(relarrow-to)$);
  \ifnum\RelationsKeyInline=1
    \node[rel key,rel key inline,anchor=mid,text=#2] at (relarrow-key) {\relkeytext{#5}};
  \else
    \node[rel key,anchor=\csname relrowanchor#6\endcsname,
      xshift=\csname relrowsign#6\endcsname\relrowgap,text=#2]
      at (relarrow-key) {\relkeytext{#5}};
  \fi
  \endgroup}
\newcommand{\relone}[5]{\relarrow{#1}{#2}{#3}{#4}{#5}{left}}
\newcommand{\relpair}[9][3.2]{%
  \path let \p1=(#2), \p2=(#3),
    \n1={#1*veclen(\x2-\x1,\y2-\y1)/abs(\y2-\y1)} in
    coordinate (relpair-A-left) at ($(\p1)+(-\n1,0)$)
    coordinate (relpair-B-left) at ($(\p2)+(-\n1,0)$)
    coordinate (relpair-A-right) at ($(\p1)+(\n1,0)$)
    coordinate (relpair-B-right) at ($(\p2)+(\n1,0)$);
  \relarrow{#4}{#5}{relpair-A-left}{relpair-B-left}{#6}{left}
  \relarrow{#7}{#8}{relpair-B-right}{relpair-A-right}{#9}{right}}


==> setup/biblio.tex <==
\providecommand{\PaperBibliographyFile}{references}
\RequirePackage{etoolbox}

\RequirePackage[
  backend=biber,
  style=authoryear,
  maxbibnames=15,
  url=false, isbn=false, doi=false,
  natbib=true, backref=true,
  uniquename=false, uniquelist=false
]{biblatex}
\DeclareCiteCommand{\citetalias}
  {\usebibmacro{prenote}}
  {\usebibmacro{citeindex}%
   \printtext[bibhyperref]{%
     \ifcsdef{abx@alias@\thefield{entrykey}}
       {\csuse{abx@alias@\thefield{entrykey}}}
       {\PackageWarning{paper-bibliography}{No alias for entry '\thefield{entrykey}'}%
        \textbf{\thefield{entrykey}}}}}
  {\multicitedelim}
  {\usebibmacro{postnote}}
\DefineBibliographyStrings{english}{%
  backrefpage = {cited on page},
  backrefpages = {cited on pages}
}
\AtEveryBibitem{%
  \clearfield{volume}%
  \clearfield{number}%
  \clearfield{pages}%
  \ifboolexpr{
    test {\iffieldequalstr{eprinttype}{arxiv}} or
    test {\iffieldequalstr{eprinttype}{arXiv}}
  }{\clearfield{howpublished}}{}%
}
\DeclareNameAlias{sortname}{given-family}
\DeclareFieldFormat*{title}{\mkbibquote{#1}}
\addbibresource{\PaperBibliographyFile.bib}
\newcommand{\PrintPaperBibliography}{\printbibliography[title={References}]}


==> setup/colors.tex <==

\RequirePackage[dvipsnames]{xcolor}

\definecolor{YaleBlue}{HTML}{00356B}
\definecolor{LinkColor}{HTML}{00356B}
\definecolor{CiteColor}{HTML}{0077BB}
\definecolor{URLColor}{HTML}{BB4444}
\definecolor{DarkRedHighlight}{HTML}{CC3311}

\definecolor{MorandiGrey}{HTML}{9B9B9B}
\definecolor{MorandiBlue}{HTML}{A3B8C1}
\definecolor{MorandiGreen}{HTML}{B2C9C2}
\definecolor{MorandiPink}{HTML}{D5C6C6}
\definecolor{MorandiBeige}{HTML}{DBCAC0}

\definecolor{fxnote}{HTML}{43AA8B}
\definecolor{fxwarning}{HTML}{F3722C}
\definecolor{fxfatal}{HTML}{F94144}



==> setup/packages.tex <==

\RequirePackage[nopatch=footnote]{microtype}

\RequirePackage{mathtools}
\RequirePackage{amsmath,amssymb,amsthm}
\RequirePackage{bm}
\RequirePackage{nicefrac}
\RequirePackage{xspace}

\RequirePackage{graphicx}
\RequirePackage{tikz}
\usetikzlibrary{arrows.meta, positioning, fit, backgrounds, decorations.markings, calc}

\RequirePackage{array}
\RequirePackage{booktabs}
\RequirePackage{pifont}
\RequirePackage{tabularx}
\RequirePackage{longtable}
\RequirePackage{multirow}
\RequirePackage{float}
\RequirePackage{wrapfig}
\RequirePackage{subcaption}
\RequirePackage{setspace}
\RequirePackage[normalem]{ulem}
\RequirePackage{outlines}
\RequirePackage{markdown}
\RequirePackage{enumitem}
\RequirePackage{colortbl}
\RequirePackage{placeins}

\setlist[itemize]{leftmargin=1.2em}

\RequirePackage{hyperref}
\RequirePackage{url}

\hypersetup{%
  colorlinks=true,
  linktocpage=true,
  pdfstartpage=1,
  pdfstartview=FitV,
  breaklinks=true,
  pdfpagemode=UseOutlines,
  pageanchor=true,
  plainpages=false,
  bookmarksnumbered,
  bookmarksopen=true,
  bookmarksopenlevel=1,
  hypertexnames=true,
  pdfhighlight=/O,
  urlcolor=Maroon,
  linkcolor=Maroon,
  citecolor=Maroon,
  pdfsubject={},
  pdfkeywords={}
}

\usepackage[capitalise,noabbrev,nameinlink]{cleveref} %

\crefname{appendix}{Appendix}{Appendices}
\Crefname{appendix}{Appendix}{Appendices}

\AddToHook{cmd/appendix/after}{%
  \crefalias{section}{appendix}%
  \crefalias{subsection}{appendix}%
  \crefalias{subsubsection}{appendix}%
}


==> setup/theory-task-matrix.tex <==
\RequirePackage{pdfrender}
\definecolor{EasyMark}{HTML}{00A63E}
\definecolor{HardMark}{HTML}{E7000B}
\definecolor{PredictionFamilyRule}{HTML}{CCCCCC}
\newcommand{\predglyphsize}{\large}
\DeclareRobustCommand{\prednewproof}{\textcolor{black}{\resizebox{!}{2.5pt}{\qedsymbol}}}
\DeclareRobustCommand{\predsymbol}[4]{%
  \mbox{%
  {\textcolor{#2}{\raisebox{-0.15ex}{\predglyphsize
    \textpdfrender{TextRenderingMode=FillStroke,LineWidth=0.2pt,StrokeColor=white}{\ding{#1}}}}}%
  \rlap{%
    \if\relax\detokenize{#3}\relax\else
      \if\relax\detokenize{#4}\relax
        \ifnum#1=55 \kern0.1pt\else\kern-0.7pt\fi
        \raisebox{4pt}{#3}%
      \else
        \ifnum#1=55 \kern0.6pt\else\kern-0.1pt\fi
        \raisebox{4.6pt}{#3}\kern0.8pt
      \fi
    \fi
    \ensuremath{{}^{\text{#4}}}}%
  }%
}
\DeclareRobustCommand{\predpos}[2][]{\predsymbol{51}{EasyMark}{#1}{#2}}
\DeclareRobustCommand{\predneg}[2][]{\predsymbol{55}{HardMark}{#1}{#2}}
\DeclareRobustCommand{\prednegc}[2][]{\predsymbol{55}{HardMark}{#1}{\ensuremath{*}#2}}
\DeclareRobustCommand{\prednone}{\textemdash}
\newcommand{\predfamilyrule}{%
  \arrayrulecolor{PredictionFamilyRule}%
  \specialrule{0.25pt}{1.375pt}{1.375pt}%
  \arrayrulecolor{black}%
}
\newcommand{\predmixedclip}{%
  (0.16,1.08) -- (0.25,0.93) -- (0.288,0.904)
  -- plot[smooth, tension=0.4] coordinates {(0.288,0.904) (0.368,0.742) (0.452,0.578) (0.543,0.456) (0.609,0.369) (0.748,0.194)}
  -- (0.70,0.12) -- (0.66,0.00) -- (0.96,0.00) -- (0.846,0.281)
  -- plot[smooth, tension=0.4] coordinates {(0.846,0.281) (0.765,0.431) (0.663,0.595) (0.558,0.750) (0.432,0.960)}
  -- (0.47,1.08) -- cycle}
\newsavebox{\predmixedcheck}
\newsavebox{\predmixedcross}
\newlength{\predmixedwidth}
\newlength{\predmixedheight}
\newlength{\predmixeddepth}
\DeclareRobustCommand{\predmixed}{%
  \sbox{\predmixedcheck}{\predpos{}}%
  \sbox{\predmixedcross}{\predneg{}}%
  \setlength{\predmixedwidth}{\wd\predmixedcross}%
  \setlength{\predmixeddepth}{\dp\predmixedcross}%
  \setlength{\predmixedheight}{\dimexpr\ht\predmixedcross+\dp\predmixedcross\relax}%
  \mbox{\usebox{\predmixedcheck}\llap{\makebox[\wd\predmixedcheck][c]{\kern-1pt%
    \tikz[baseline=0pt]{%
    \useasboundingbox (0,0) rectangle (\predmixedwidth,0);
    \begin{scope}
      \clip[x=\predmixedwidth, y=\predmixedheight, yshift=-\predmixeddepth, xscale=1.12, xshift=-0.06\predmixedwidth] \predmixedclip;
      \node[inner sep=0, anchor=base west] at (0,0) {\raisebox{-0.15ex}{\predglyphsize
        \textpdfrender{TextRenderingMode=FillStroke,LineWidth=1.2pt,StrokeColor=white,FillColor=white}{\ding{55}}}};
    \end{scope}
    \begin{scope}
      \clip[x=\predmixedwidth, y=\predmixedheight, yshift=-\predmixeddepth] \predmixedclip;
      \node[inner sep=0, anchor=base west] at (0,0) {\usebox{\predmixedcross}};
    \end{scope}}}}}%
}
\definecolor{PredictionDisagreeTint}{HTML}{FBE3E1}
\ifx\AgreementBars\undefined\def\AgreementBars{2}\fi%
\ifx\AgreementFadeSensitivity\undefined\def\AgreementFadeSensitivity{0}\fi%
\ifx\AgreementSensitivityDenominator\undefined\def\AgreementSensitivityDenominator{1}\fi%
\ifx\AgreementRowDenominator\undefined\def\AgreementRowDenominator{1}\fi%
\definecolor{AgreementAllColor}{HTML}{4A6C8C}
\definecolor{AgreementDenominatorGray}{HTML}{8C8C8C}
\newcommand{\predagreementstrengths}[1]{%
  \ifnum#1=1
    \def\predagreementsolid{40}\def\predagreementborder{50}\def\predagreementlight{6}%
    \def\predagreementtextcolor{AgreementDenominatorGray}%
  \else
    \def\predagreementsolid{80}\def\predagreementborder{85}\def\predagreementlight{12}%
    \def\predagreementtextcolor{black}%
  \fi}
\newcommand{\predagreementsegment}[6]{%
  \ifnum#4>0
    \fill[#1!\predagreementlight] (#2pt,#5pt) rectangle ({#2pt+#4pt},#6pt);
    \ifnum#3>0 \fill[#1!\predagreementsolid] (#2pt,#5pt) rectangle ({#2pt+#3pt},#6pt);\fi
    \draw[#1!\predagreementborder, line width=0.3pt]
      ({#2pt+0.15pt},{#5pt+0.15pt}) rectangle ({#2pt+#4pt-0.15pt},{#6pt-0.15pt});
  \fi}
\newcommand{\predagreementtotal}[4]{%
  \ifnum\numexpr\predagreementrowtotal-#2\relax>0
    \fill[white] (#2pt,#3pt) rectangle (\predagreementrowtotal pt,#4pt);
    \draw[#1!\predagreementborder, line width=0.3pt]
      ({#2pt+0.15pt},{#3pt+0.15pt}) rectangle ({\predagreementrowtotal pt-0.15pt},{#4pt-0.15pt});
  \fi}
\gdef\predagreementrowtotal{0}
\newcommand{\predagreementbars}[4]{%
  \tikz[baseline=0pt]{%
    \ifcase\AgreementBars\or
      \predagreementsegment{AgreementAllColor}{0}{\the\numexpr#1+#3\relax}{\the\numexpr#2+#4\relax}{0.1}{5.1}
      \predagreementtotal{AgreementAllColor}{\the\numexpr#2+#4\relax}{0.1}{5.1}
    \or
      \predagreementsegment{AgreementAllColor}{0}{\the\numexpr#1+#3\relax}{\the\numexpr#2+#4\relax}{3.05}{7.45}
      \predagreementtotal{AgreementAllColor}{\the\numexpr#2+#4\relax}{3.05}{7.45}
      \predagreementsegment{TaskEasyColor}{0}{#1}{#2}{-2.25}{2.15}
      \predagreementsegment{TaskHardColor}{#2}{#3}{#4}{-2.25}{2.15}
    \or
      \predagreementsegment{TaskEasyColor}{0}{#1}{#2}{0.1}{5.1}
      \predagreementsegment{TaskHardColor}{#2}{#3}{#4}{0.1}{5.1}
      \predagreementtotal{black}{\the\numexpr#2+#4\relax}{0.1}{5.1}
    \fi}}
\newcommand{\predagreementcell}[8]{%
  \begingroup
  \predagreementstrengths{\the\numexpr#5*\AgreementFadeSensitivity\relax}%
  \edef\predagreementcount{\the\numexpr#1+#3\relax}%
  \edef\predagreementscored{\the\numexpr#2+#4\relax}%
  \ifnum\AgreementBars=0
    \textcolor{\predagreementtextcolor}{\predagreementcount/\predagreementscored}%
  \else
    {\scriptsize\hphantom{#6}\llap{\textcolor{\predagreementtextcolor}{\predagreementcount}}}\,%
    \makebox[\ifnum\predagreementrowtotal>#7 \predagreementrowtotal\else#7\fi pt][l]{\predagreementbars{#1}{#2}{#3}{#4}}%
    \ifnum\AgreementSensitivityDenominator=1
      \if\relax\detokenize{#8}\relax\else
        \hspace{1.8pt}{\fontsize{5.5}{6}\selectfont\color{AgreementDenominatorGray}%
          \rlap{\ifnum#5=1 (of \predagreementscored)\fi}\hphantom{#8}}%
      \fi
    \fi
  \fi
  \endgroup}
\newcommand{\predagreementlabel}[2]{%
  \gdef\predagreementrowtotal{#2}%
  \quad #1%
  \ifnum\AgreementRowDenominator=1
    \ifnum\AgreementBars>0 \space\textcolor{AgreementDenominatorGray}{(of #2)}\fi
  \fi}
\newcommand{\predagreementrowskip}{\ifnum\AgreementBars=2 2.5pt\else 0pt\fi}
\newcommand{\predagreementswatchbox}[2]{\tikz[baseline=-0.3pt]{%
  \fill[#1] (0,0) rectangle (5pt,4.5pt);
  \draw[#2, line width=0.3pt] (0.15pt,0.15pt) rectangle (4.85pt,4.35pt);}}
\newcommand{\predagreementswatch}[1]{\predagreementswatchbox{#1!80}{#1!85}}
\newcommand{\predagreementframe}[1][PredAgreementLight]{%
  \ifnum\AgreementBars=3
    \colorlet{PredAgreementOutline}{black!85}\colorlet{PredAgreementLight}{black!10}%
  \else
    \colorlet{PredAgreementOutline}{AgreementAllColor!85}\colorlet{PredAgreementLight}{AgreementAllColor!12}%
  \fi
  \predagreementswatchbox{#1}{PredAgreementOutline}}
\newcommand{\predagreementlegendall}{%
  \predagreementswatch{AgreementAllColor} & agree\\[-1.5pt]}
\newcommand{\predagreementlegendsplit}{%
  \multicolumn{2}{@{}l@{}}{\textcolor{AgreementAllColor}{All}/\textcolor{TaskEasyColor}{Easy}/\textcolor{TaskHardColor}{Hard}}\\[-1.5pt]
  \predagreementswatch{AgreementAllColor}\,\predagreementswatch{TaskEasyColor}\,\predagreementswatch{TaskHardColor} & agree\\[-1.5pt]}
\newcommand{\predagreementlegendstacked}{%
  \multicolumn{2}{@{}l@{}}{\textcolor{TaskEasyColor}{Easy}\,/\,\textcolor{TaskHardColor}{Hard}}\\[-1.5pt]
  \predagreementswatch{TaskEasyColor}\,\predagreementswatch{TaskHardColor} & agree\\[-1.5pt]}
\newcommand{\predagreementlegend}{%
  \ifnum\AgreementBars>0
    \ifcase\AgreementBars\or
      \let\predagreementlegendrows\predagreementlegendall
    \or
      \let\predagreementlegendrows\predagreementlegendsplit
    \or
      \let\predagreementlegendrows\predagreementlegendstacked
    \fi
    \hspace{2pt}\smash{\scriptsize
      \begin{tabular}[c]{@{}l@{\,}l@{}}
        \predagreementlegendrows
        \predagreementframe & disagree\\[-1.5pt]
        \predagreementframe[white] & n/a
      \end{tabular}}%
  \fi}

